In Situ Translational Hand-Eye Calibration of Laser Profile Sensors using Arbitrary Objects

Hand-eye calibration of laser profile sensors is the process of extracting the homogeneous transformation between the laser profile sensor frame and the end-effector frame of a robot in order to express the data extracted by the sensor in the robot's global coordinate system. For laser profile scanners this is a challenging procedure, as they provide data only in two dimensions and state-of-the-art calibration procedures require the use of specialised calibration targets. This paper presents a novel method to extract the translation-part of the hand-eye calibration matrix with rotation-part known a priori in a target-agnostic way. Our methodology is applicable to any 2D image or 3D object as a calibration target and can also be performed in situ in the final application. The method is experimentally validated on a real robot-sensor setup with 2D and 3D targets.

==> leftovers.tex <==

%\todo[inline]{ST: Let's use decide if we 2D or 2D, and let's stick to it.}


% \textcolor{red}{The point cloud considered in this section is the one obtained after the segmentation process which is different in the case of 2D and 3D objects and is detailed in Section \ref{subsec:data_acquisition}. After segmentation, the method presented in this section is valid for both cases of 2D or 3D object scans. The transformation from 2D points expressed in the sensor frame into the 3D points expressed in the base frame is done by using an homogeneous transformation matrix ${}^E H_S$ between the sensor coordinate system $S$ and the end-effector coordinate system $E$. It is defined as:
% }
% \todo[inline]{ST: I do not like that we refer to the experimenta section, I will try to provide some suggestions to IS.}
% \todo[inline]{ST: I will simplify this section.}
